FastMask: Segment Multi-scale Object Candidates in One Shot

Objects appear to scale differently in natural images. This fact requires methods dealing with object-centric tasks (e.g. object proposal) to have robust performance over variances in object scales. In the paper, we present a novel segment proposal framework, namely FastMask, which takes advantage of hierarchical features in deep convolutional neural networks to segment multi-scale objects in one shot. Innovatively, we adapt segment proposal network into three different functional components (body, neck and head). We further propose a weight-shared residual neck module as well as a scale-tolerant attentional head module for efficient one-shot inference. On MS COCO benchmark, the proposed FastMask outperforms all state-of-the-art segment proposal methods in average recall being 2~5 times faster. Moreover, with a slight trade-off in accuracy, FastMask can segment objects in near real time (~13 fps) with 800*600 resolution images, demonstrating its potential in practical applications. Our implementation is available on https://github.com/voidrank/FastMask.

==> main <==
\begin{thebibliography}{10}\itemsep=-1pt

\bibitem{arbelaez_cvpr14}
P.~Arbel{\'a}ez, J.~Pont-Tuset, J.~T. Barron, F.~Marques, and J.~Malik.
\newblock Multiscale combinatorial grouping.
\newblock In {\em CVPR}, 2014.

\bibitem{bell_cvpr16}
S.~Bell, C.~L. Zitnick, K.~Bala, and R.~Girshick.
\newblock Inside-outside net: Detecting objects in context with skip pooling
  and recurrent neural networks.
\newblock In {\em CVPR}, 2016.

\bibitem{chen_iclr15}
L.-C. Chen, G.~Papandreou, I.~Kokkinos, K.~Murphy, and A.~L. Yuille.
\newblock Semantic image segmentation with deep convolutional nets and fully
  connected crfs.
\newblock In {\em ICLR}, 2015.

\bibitem{cheng_cvpr14}
M.-M. Cheng, Z.~Zhang, W.-Y. Lin, and P.~Torr.
\newblock Bing: Binarized normed gradients for objectness estimation at 300fps.
\newblock In {\em CVPR}, 2014.

\bibitem{dai_eccv16}
J.~Dai, K.~He, Y.~Li, S.~Ren, and J.~Sun.
\newblock Instance-sensitive fully convolutional networks.
\newblock In {\em ECCV}, 2016.

\bibitem{dai_cvpr16}
J.~Dai, K.~He, and J.~Sun.
\newblock Instance-aware semantic segmentation via multi-task network cascades.
\newblock In {\em CVPR}, 2016.

\bibitem{erhan_cvpr14}
D.~Erhan, C.~Szegedy, A.~Toshev, and D.~Anguelov.
\newblock Scalable object detection using deep neural networks.
\newblock In {\em CVPR}, 2014.

\bibitem{girshick_cvpr14}
R.~Girshick, J.~Donahue, T.~Darrell, and J.~Malik.
\newblock Rich feature hierarchies for accurate object detection and semantic
  segmentation.
\newblock In {\em CVPR}, 2014.

\bibitem{girshick_cvpr15}
R.~Girshick, F.~Iandola, T.~Darrell, and J.~Malik.
\newblock Deformable part models are convolutional neural networks.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 437--446, 2015.

\bibitem{gokberk_cvpr13}
R.~Gokberk~Cinbis, J.~Verbeek, and C.~Schmid.
\newblock Segmentation driven object detection with fisher vectors.
\newblock In {\em CVPR}, 2013.

\bibitem{habriharan_eccv14}
B.~Hariharan, P.~Arbel{\'a}ez, R.~Girshick, and J.~Malik.
\newblock Simultaneous detection and segmentation.
\newblock In {\em ECCV}, 2014.

\bibitem{he_cvpr16}
K.~He, X.~Zhang, S.~Ren, and J.~Sun.
\newblock Deep residual learning for image recognition.
\newblock In {\em CVPR}, 2016.

\bibitem{he_eccv16}
K.~He, X.~Zhang, S.~Ren, and J.~Sun.
\newblock Identity mappings in deep residual networks.
\newblock In {\em ECCV}, 2016.

\bibitem{kim_arxiv16}
S.~Hong, B.~Roh, K.-H. Kim, Y.~Cheon, and M.~Park.
\newblock Pvanet: Lightweight deep neural networks for real-time object
  detection.
\newblock {\em arXiv preprint arXiv:1611.08588}, 2016.

\bibitem{hosang_pami16}
J.~Hosang, R.~Benenson, P.~Doll{\'a}r, and B.~Schiele.
\newblock What makes for effective detection proposals?
\newblock {\em IEEE T-PAMI}, 2016.

\bibitem{krahenbuhl_eccv14}
P.~Kr{\"a}henb{\"u}hl and V.~Koltun.
\newblock Geodesic object proposals.
\newblock In {\em ECCV}, 2014.

\bibitem{kuo_iccv15}
W.~Kuo, B.~Hariharan, and J.~Malik.
\newblock Deepbox: Learning objectness with convolutional networks.
\newblock In {\em ICCV}, 2015.

\bibitem{lin_eccv14}
T.-Y. Lin, M.~Maire, S.~Belongie, J.~Hays, P.~Perona, D.~Ramanan,
  P.~Doll{\'a}r, and C.~L. Zitnick.
\newblock Microsoft coco: Common objects in context.
\newblock In {\em ECCV}, 2014.

\bibitem{liu_arxiv2016}
C.~Liu, J.~Mao, F.~Sha, and A.~Yuille.
\newblock Attention correctness in neural image captioning.
\newblock {\em arXiv preprint arXiv:1605.09553}, 2016.

\bibitem{pinheiro_nips15}
P.~O. Pinheiro, R.~Collobert, and P.~Dollar.
\newblock Learning to segment object candidates.
\newblock In {\em NIPS}, 2015.

\bibitem{pinheiro_eccv16}
P.~O. Pinheiro, T.-Y. Lin, R.~Collobert, and P.~Doll{\'a}r.
\newblock Learning to refine object segments.
\newblock In {\em ECCV}, 2016.

\bibitem{ren_nips15}
S.~Ren, K.~He, R.~Girshick, and J.~Sun.
\newblock Faster r-cnn: Towards real-time object detection with region proposal
  networks.
\newblock In {\em NIPS}, 2015.

\bibitem{shelhamer_pami16}
E.~Shelhamer, J.~Long, and T.~Darrell.
\newblock Fully convolutional networks for semantic segmentation.
\newblock {\em IEEE T-PAMI}, 2016.

\bibitem{simonyan_iclr15}
K.~Simonyan and A.~Zisserman.
\newblock Very deep convolutional networks for large-scale image recognition.
\newblock In {\em ICLR}, 2015.

\bibitem{van_iccv11}
K.~E. Van~de Sande, J.~R. Uijlings, T.~Gevers, and A.~W. Smeulders.
\newblock Segmentation as selective search for object recognition.
\newblock In {\em ICCV}. IEEE, 2011.

\bibitem{xu_icml15}
K.~Xu, J.~Ba, R.~Kiros, K.~Cho, A.~Courville, R.~Salakhutdinov, R.~S. Zemel,
  and Y.~Bengio.
\newblock Show, attend and tell: Neural image caption generation with visual
  attention.
\newblock In {\em ICML}, 2015.

\bibitem{yang_cvpr2016}
Z.~Yang, X.~He, J.~Gao, L.~Deng, and A.~Smola.
\newblock Stacked attention networks for image question answering.
\newblock 2016.

\bibitem{yu_iclr16}
F.~Yu and V.~Koltun.
\newblock Multi-scale context aggregation by dilated convolutions.
\newblock In {\em ICLR}, 2016.

\bibitem{zhang_cvpr11}
Z.~Zhang, J.~Warrell, and P.~H. Torr.
\newblock Proposal generation for object detection using cascaded ranking svms.
\newblock In {\em CVPR}, 2011.

\bibitem{zhu_cvpr16}
Y.~Zhu, O.~Groth, M.~Bernstein, and L.~Fei-Fei.
\newblock Visual7w: Grounded question answering in images.
\newblock 2016.

\bibitem{zitnick_eccv14}
C.~L. Zitnick and P.~Doll{\'a}r.
\newblock Edge boxes: Locating object proposals from edges.
\newblock In {\em ECCV}, 2014.

\end{thebibliography}

